Phoenix: Democratizing ChatGPT across Languages

This paper presents our efforts to democratize ChatGPT across language. We release a large language model "Phoenix", achieving competitive performance among open-source English and Chinese models while excelling in languages with limited resources (covering both Latin and non-Latin languages). We believe this work will be beneficial to make ChatGPT more accessible, especially in countries where people cannot use ChatGPT due to restrictions from OpenAI or local goverments. Our data, code, and models are available at https://github.com/FreedomIntelligence/LLMZoo.

==> mybibitem.tex <==
\begin{thebibliography}{200}
\bibitem{notes} John W. Dower \emph{Readings compiled for History 21.479.} 1991.
\bibitem{impj}  The Japan Reader \emph{Imperial Japan 1800-1945} 1973: Random House, N.Y.
\end{thebibliography}

